The Quasar Catalogue for S-PLUS DR4 (QuCatS) and the estimation of photometric redshifts

The advent of massive broad-band photometric surveys enabled photometric redshift estimates for unprecedented numbers of galaxies and quasars. These estimates can be improved using better algorithms or by obtaining complementary data such as narrow-band photometry, and broad-band photometry over an extended wavelength range. We investigate the impact of both approaches on photometric redshifts for quasars using data from Southern Photometric Local Universe Survey (S-PLUS) DR4, Galaxy Evolution Explorer (GALEX) DR6/7, and the unWISE catalog for the Wide-field Infrared Survey Explorer (WISE) in three machine learning methods: Random Forest, Flexible Conditional Density Estimation (FlexCoDE), and Bayesian Mixture Density Network (BMDN). Including narrow-band photometry improves the root-mean-square error by 11% in comparison to a model trained with only broad-band photometry. Narrow-band information only provided an improvement of 3.8% when GALEX and WISE colours were included. Thus narrow bands play a more important role for objects that do not have GALEX or WISE counterparts, which respectively makes 92% and 25% of S-PLUS data considered here. Nevertheless, the inclusion of narrow-band information provided better estimates of the probability density functions obtained with FlexCoDE and BMDN. We publicly release a value-added catalogue of photometrically selected quasars with the photo-z predictions from all methods studied here. The catalogue provided with this work covers the S-PLUS DR4 area (~3000deg$^2$), containing 645 980, 244 912, 144 991 sources with the probability of being a quasar higher than, 80%, 90%, 95% up to r < 21.3 and good photometry quality in the detection image. More quasar candidates can be retrieved from the S-PLUS data base by considering less restrictive selection criteria.

==> tex/fig/J0861-W2xJ0515-i.tex <==
\begin{figure}
    \includegraphics[width=0.5\textwidth]{fig/J0861-W2xJ0515-i.png}
  \caption{Colour-colour diagram (J0515-i versus J0861-W2) for all spectroscopic confirmed quasars from our sample, coloured by their spectroscopic redshift. }
    \label{fig:colorcolor}
\end{figure}

==> tex/fig/metrics_old.tex <==
\begin{figure*}
\centering
\subfloat[]{\includegraphics[width=0.30\textwidth]{fig/rmse_r_PStotal.png}
\label{pre:a}}
\hfil
\subfloat[]{\includegraphics[width=0.30\textwidth]{fig/rmse_g-r.png}%
\label{pre:b}}
\hfil
\subfloat[]{\includegraphics[width=0.30\textwidth]{fig/rmse_Z.png}%
\label{pre:c}}
\hfil

\centering
\subfloat[]{\includegraphics[width=0.30\textwidth]{fig/sigma_r_PStotal.png}
\label{pre:d}}
\hfil
\subfloat[]{\includegraphics[width=0.30\textwidth]{fig/sigma_g-r.png}%
\label{pre:e}}
\hfil
\subfloat[]{\includegraphics[width=0.30\textwidth]{fig/sigma_Z.png}%
\label{pre:f}}
\hfil

\centering
\subfloat[]{\includegraphics[width=0.30\textwidth]{fig/bias_r_PStotal.png}%
\label{pre:g}}
\hfil
\subfloat[]{\includegraphics[width=0.30\textwidth]{fig/bias_g-r.png}%
\label{pre:h}}
\hfil
\subfloat[]{\includegraphics[width=0.30\textwidth]{fig/bias_Z.png}%
\label{pre:i}}
\hfil

\centering
\subfloat[]{\includegraphics[width=0.30\textwidth]{fig/out_frac_r_PStotal.png}%
\label{pre:j}}
\hfil
\subfloat[]{\includegraphics[width=0.30\textwidth]{fig/out_frac_g-r.png}%
\label{pre:k}}
\hfil
\subfloat[]{\includegraphics[width=0.30\textwidth]{fig/out_frac_Z.png}%
\label{pre:l}}
\hfil

\caption{Performance of the model broad (blue) and broad+narrow+galex+wise (pink) from cross-validation. Curves are given by the median $\pm$ 1$\sigma$ of the metrics measured for each fold.  (a) RMSE per magnitude r; (b) RMSE per colour g-r; (c) RMSE per spectroscopic redshift; (d) NMAD per magnitude r; (e) NMAD per colour g-r; (f) NMAD per spectroscopic redshift; (g) Bias per magnitude r; (h) Bias per colour g-r; (i) Bias per spectroscopic redshift; (j) $\eta_{0.30}$ per magnitude r; (h) $\eta_{0.30}$ per colour g-r; (l) $\eta_{0.30}$ per spectroscopic redshift.}
\vspace{-10 pt}  % adjust the vertical spacing
\label{fig:metrics}
\end{figure*}




\begin{figure*}
    \subfloat[]{\includegraphics[width=0.32\textwidth]{fig/997_scatter_z_per_r_lim20.png}}
        \subfloat[]{\includegraphics[width=0.32\textwidth]{fig/997_scatter_z_per_r_lim21.png}}
             \subfloat[]{\includegraphics[width=0.32\textwidth]{fig/997_scatter_z_per_r_lim22.png}}
  \caption{Photometric redshifts estimated by model \textcolor{red}{997} (top panels) and residuals (bottom panels) per spectroscopic redshifts. Left, middle and right panels are shown to facilitate the visualization of the data, limited to: (a) $r$ < 20; (b) $r$ < 21; (c) $r$ < 22. \textcolor{red}{only plot a small interval and use color for density because the other figure of sigma already has the same information. DO another plot r x g-i and colored by spectroscopic redshift. Include another plot histogram delta z (z with narrow bands - z without narrow bands)}}
    \label{fig:bxl}
\end{figure*}

==> tex/fig/vac_r.tex <==
\begin{figure*}
    \includegraphics[width=0.8\textwidth]{fig/vac/hist_r_qsos.png}
  \caption{Colour-colour diagram (J0515-i versus J0861-W2) for all spectroscopic confirmed quasars from our sample, coloured by their spectroscopic redshift. }
    \label{fig:vac_r}
\end{figure*}

==> tex/table/test2.tex <==
\begin{table*}
\begin{tabular}{@{}lllllll@{}}
\toprule
& Feature Space & \multicolumn{1}{c}{$\sigma_{\text{RMSE}}$} & \multicolumn{1}{c}{$\sigma_{\text{NMAD}}$} & \multicolumn{1}{c}{$\mu$}
& \multicolumn{1}{c}{$\eta_{0.15}$} & \multicolumn{1}{c}{$\eta_{0.30}$} \\\midrule
{Random Forest}                    & Without narrow bands & 3.9 & 7.8  & -2.3 & 5.2 & 4.7     \\\midrule
{FlexCoDE}                         & Without narrow bands & 5.2 & 52.3 & 63.0 & 8.8 & 5.4   \\\midrule
{Bayesian Mixture Density Network} & Without narrow bands & 6.2 & 40.4 & 51.4 & 9.1 & 14.9    \\\midrule
{Average}                          & Without narrow bands & 6.7 & 29.7 & 76.9 & 8.7 & 12.3    \\\bottomrule
\end{tabular}
\end{table*}
